When the Ground Truth is not True: Modelling Human Biases in Temporal Annotations

In supervised learning, low quality annotations lead to poorly performing classification and detection models, while also rendering evaluation unreliable. This is particularly apparent on temporal data, where annotation quality is affected by multiple factors. For example, in the post-hoc self-reporting of daily activities, cognitive biases are one of the most common ingredients. In particular, reporting the start and duration of an activity after its finalisation may incorporate biases introduced by personal time perceptions, as well as the imprecision and lack of granularity due to time rounding. Here we propose a method to model human biases on temporal annotations and argue for the use of soft labels. Experimental results in synthetic data show that soft labels provide a better approximation of the ground truth for several metrics. We showcase the method on a real dataset of daily activities.

==> figures/tikz_annotation_examples.tex <==
\begin{tikzpicture}
\tikzset{x=0.75ex, y=0.75ex} % MPN: Change the scale

% Annotation A
\draw[draw=lightgray, fill=teal!30] (0, 20) rectangle ++(60, 6) node[pos=.5] {A: 1h annotation};
\draw [->] (0, 20) -- (60, 20); % X axis
\draw [->] (0, 20) -- (0, 28); % Y axis
\draw [|-|] (0, 26) -- (10, 26)
  node[pos=0.5, anchor=south] {A:FP}; % Top text False positive
\draw [|-|] (10, 26) -- (47, 26)
  node[pos=0.5, anchor=south] {A:TP}; % Top text True positive
\draw [|-|] (47, 26) -- (60, 26)
  node[pos=0.5, anchor=south] {A:FP}; % Top text False positive
    
% Annotation B
\draw[draw=lightgray, fill=teal!30] (0, 10) rectangle ++(30, 6) node[pos=.5] {B: 30min. annot.};
\draw[draw=blue!60, densely dotted]  (15, 16) -- (45, 10)
  node[text=blue!60, pos=.5, anchor=south west] at ++(10, 10)
    {soft label}; % Soft label right
\draw [draw=blue!60, densely dotted]  (0, 14) -- (15, 16); % Soft label left
\draw [->] (0, 10) -- (60, 10); % X axis
\draw [->] (0, 10) -- (0, 18); % Y axis
\draw [|-|] (0, 16) -- (10, 16)
  node[pos=0.5, anchor=south] {B:FP}; % Top text False positive
\draw [|-|] (10, 16) -- (30, 16)
  node[pos=0.5, anchor=south] {B:TP}; % Top text True positive
\draw [|-|] (30, 16) -- (47, 16)
  node[pos=0.5, anchor=south] {B:FN}; % Top text True positive
\draw [|-|] (47, 16) -- (60, 16)
  node[pos=0.5, anchor=south] {B:TN}; % Top text False positive
    
% Ground Truth
\draw[draw=lightgray, fill=red!30] (10, 0) rectangle ++(37, 6) node[pos=.5] {Ground Truth: 37min. shower};
\draw [->] (0, 0) -- (60, 0); % X axis
\draw [->] (0, 0) -- (0, 8); % Y axis

\node [] at (0, -2) {8am};
\node [] at (30, -2) {8:30am};
\node [] at (60, -2) {9am};

\draw [dotted] (10, -1) -- (10, 30)
  node[pos=0, anchor=north] {$d_0^*$}; % Vertical line start shower
\draw [dotted] (47, -1) -- (47, 30)
  node[pos=0, anchor=north] {$d_1^*$}; % Vertical line end shower
\end{tikzpicture}

==> figures/tikz_signal_uncertainties.tex <==
\begin{tikzpicture}
\draw [->] (-4.2,-0.3) -- (-4.2,2);
\draw [->] (-4.2,-0.3) -- (2,-0.3);
\node[rectangle,
    draw = lightgray,
    text = olive,
    fill = teal!30!white,
    minimum width = 2cm, 
    minimum height = 2cm] (r) at (-2,0.8) {};
 
\path [draw=blue,snakeline]  (-4,0) -- (2,0);
\node [teal] at (-3,2) {$l_0$};
\node [teal] at (-1,2) {$l_1$};
\node [] at (1.2,0.2) {$signal$};
\node [] at (1.9,-0.5) {$t$};
\draw [densely dotted] (-2,-0.3) -- (-2,2);  
\node [] at (-2,2) {$l_s$};
\draw [densely dotted] (-1.68,-0.3) -- (-1.68,0.65);  
\draw [densely dotted] (-1.1,-0.3) -- (-1.1,0.65);  
\node [] at (-1.7,-.5) {$e_0$};
\node [] at (-1.1,-0.5) {$e_1$};
\end{tikzpicture}
